Unsupervised Co-Learning on $\mathcal{G}$-Manifolds Across Irreducible Representations

We introduce a novel co-learning paradigm for manifolds naturally equipped with a group action, motivated by recent developments on learning a manifold from attached fibre bundle structures. We utilize a representation theoretic mechanism that canonically associates multiple independent vector bundles over a common base manifold, which provides multiple views for the geometry of the underlying manifold. The consistency across these fibre bundles provide a common base for performing unsupervised manifold co-learning through the redundancy created artificially across irreducible representations of the transformation group. We demonstrate the efficacy of the proposed algorithmic paradigm through drastically improved robust nearest neighbor search and community detection on rotation-invariant cryo-electron microscopy image analysis.

==> textfiles/other_materials.tex <==

To visualize the clustering results of $K = 10$, in Figs.~\ref{fig:10_cluster_plot_SO2} and~\ref{fig:10_cluster_plot_SO3}, we show the coloring of the clusters in the 2-D scatter plots of the data (clustering accuracies are shown in the main paper), with $\SO(2)$ and $\SO(3)$ group transformations. 
We generate the scatter plots by first assigning the coordinates for each data point on the 2-D plane (these coordinates are used for visualization and not used for the initial clean graph generation). 
The top rows of Figs.~\ref{fig:10_cluster_plot_SO2} and~\ref{fig:10_cluster_plot_SO3} show the ground truth coloring of the points based on the clean graphs. 
For noisy graphs, we assign colors based on the clustering results by each affinity measure (the ordering of the colors may vary from plot to plot). Visually, our proposed affinities achieve more accurate clustering than vector diffusion maps (VDM)~\cite{SingerWu2012VDM} and traditional spectral clustering~\cite{ng2002spectral}, with less mixing colors within individual clusters. 
\begin{figure}[htb!]
     \centering
     \setlength\tabcolsep{0.1pt}
     \renewcommand{\arraystretch}{0.8}
     \begin{tabular}{ p{0.03\textwidth}<{\centering} p{0.18\textwidth}<{\centering} p{0.18\textwidth}<{\centering} p{0.18\textwidth}<{\centering} p{0.18\textwidth}<{\centering}  p{0.18\textwidth}<{\centering}}
     & \multicolumn{5}{c}{\scriptsize{\quad \textbf{Ground truth}}}\\[4pt]
     & \multicolumn{5}{c}{\includegraphics[width = 0.18\textwidth]{figures/Spectral_clustering/10cluster/gt16_K_10_m_10_kmax_10.eps}}\\[5pt]
     &\scriptsize{\quad Scalar } &\scriptsize{\quad VDM} &\scriptsize{\quad \textbf{Power spec. (ours)}} &\scriptsize{\quad \textbf{Opt (ours)}} &\scriptsize{\quad \textbf{Bispec. (ours)}}\\[-12pt]
     \raisebox{-2.5\height}{\rotatebox{90}{\textbf{\scriptsize{p = 0.25}}}}
     &\subfloat{\includegraphics[width = 0.18\textwidth]{figures/Spectral_clustering/10cluster/Spectral_clus_0_25.eps}}
     &\subfloat{\includegraphics[width = 0.18\textwidth]{figures/Spectral_clustering/10cluster/VDM0_25.eps}}
     &\subfloat{\includegraphics[width = 0.18\textwidth]{figures/Spectral_clustering/10cluster/Power_spec_0_25.eps}}
     &\subfloat{\includegraphics[width = 0.18\textwidth]{figures/Spectral_clustering/10cluster/Opt0_25.eps}}
     &\subfloat{\includegraphics[width = 0.18\textwidth]{figures/Spectral_clustering/10cluster/Bispec_0_25.eps}}
     \\[-12pt]
     \raisebox{-2.5\height}{\rotatebox{90}{\textbf{\scriptsize{p = 0.20}}}}
     &\subfloat{\includegraphics[width = 0.18\textwidth]{figures/Spectral_clustering/10cluster/Spectral_clus_0_20.eps}}
     &\subfloat{\includegraphics[width = 0.18\textwidth]{figures/Spectral_clustering/10cluster/VDM0_20.eps}}
     &\subfloat{\includegraphics[width = 0.18\textwidth]{figures/Spectral_clustering/10cluster/Power_spec_0_20.eps}}
     &\subfloat{\includegraphics[width = 0.18\textwidth]{figures/Spectral_clustering/10cluster/Opt0_20.eps}}
     &\subfloat{\includegraphics[width = 0.18\textwidth]{figures/Spectral_clustering/10cluster/Bispec_0_20.eps}}\\[-12pt]
     \raisebox{-2.5\height}{\rotatebox{90}{\textbf{\scriptsize{p = 0.16}}}}
     &\subfloat{\includegraphics[width = 0.18\textwidth]{figures/Spectral_clustering/10cluster/Spectral_clus_0_16.eps}}
     &\subfloat{\includegraphics[width = 0.18\textwidth]{figures/Spectral_clustering/10cluster/VDM0_16.eps}}
     &\subfloat{\includegraphics[width = 0.18\textwidth]{figures/Spectral_clustering/10cluster/Power_spec_0_16.eps}}
     &\subfloat{\includegraphics[width = 0.18\textwidth]{figures/Spectral_clustering/10cluster/Opt0_16.eps}}
     &\subfloat{\includegraphics[width = 0.18\textwidth]{figures/Spectral_clustering/10cluster/Bispec_0_16.eps}}
     \end{tabular}
     \caption{Spectral clustering result with $K = 10$ clusters and $\SO(2)$ group transformation, with different noise levels. We have $n = 500$ number of points and each cluster has 50 points.}
     \label{fig:10_cluster_plot_SO2}
\end{figure}

\begin{figure}[htb!]
     \centering
     \setlength\tabcolsep{0.1pt}
     \renewcommand{\arraystretch}{0.8}
     \begin{tabular}{ p{0.03\textwidth}<{\centering} p{0.18\textwidth}<{\centering} p{0.18\textwidth}<{\centering} p{0.18\textwidth}<{\centering} p{0.18\textwidth}<{\centering} }
     & \multicolumn{4}{c}{\scriptsize{~ \textbf{Ground truth}}}\\[-3pt]
     & \multicolumn{4}{c}{\includegraphics[width = 0.22\textwidth]{figures/Spectral_clustering/10cluster_SO3/gt16_K_10_m_10_kmax_10.eps}}\\[5pt]
     &\scriptsize{\quad Scalar.} &\scriptsize{\quad VDM.} &\scriptsize{\quad \textbf{Power spec. (ours)}} &\scriptsize{\quad \textbf{Bispec. (ours)}}\\[-12pt]
     \raisebox{-2.5\height}{\rotatebox{90}{\textbf{\scriptsize{p = 0.25}}}}
     &\subfloat{\includegraphics[width = 0.18\textwidth]{figures/Spectral_clustering/10cluster_SO3/Spectral_clus_0_25.eps}}
     &\subfloat{\includegraphics[width = 0.18\textwidth]{figures/Spectral_clustering/10cluster_SO3/VDM0_25.eps}}
     &\subfloat{\includegraphics[width = 0.18\textwidth]{figures/Spectral_clustering/10cluster_SO3/Power_spec_0_25.eps}}
     &\subfloat{\includegraphics[width = 0.18\textwidth]{figures/Spectral_clustering/10cluster_SO3/Bispec_0_25.eps}}
     \\[-12pt]
     \raisebox{-2.5\height}{\rotatebox{90}{\textbf{\scriptsize{p = 0.20}}}}
     &\subfloat{\includegraphics[width = 0.18\textwidth]{figures/Spectral_clustering/10cluster_SO3/Spectral_clus_0_20.eps}}
     &\subfloat{\includegraphics[width = 0.18\textwidth]{figures/Spectral_clustering/10cluster_SO3/VDM0_20.eps}}
     &\subfloat{\includegraphics[width = 0.18\textwidth]{figures/Spectral_clustering/10cluster_SO3/Power_spec_0_20.eps}}
     &\subfloat{\includegraphics[width = 0.18\textwidth]{figures/Spectral_clustering/10cluster_SO3/Bispec_0_20.eps}}\\[-12pt]
     \raisebox{-2.5\height}{\rotatebox{90}{\textbf{\scriptsize{p = 0.16}}}}
     &\subfloat{\includegraphics[width = 0.18\textwidth]{figures/Spectral_clustering/10cluster_SO3/Spectral_clus_0_16.eps}}
     &\subfloat{\includegraphics[width = 0.18\textwidth]{figures/Spectral_clustering/10cluster_SO3/VDM0_16.eps}}
     &\subfloat{\includegraphics[width = 0.18\textwidth]{figures/Spectral_clustering/10cluster_SO3/Power_spec_0_16.eps}}
     &\subfloat{\includegraphics[width = 0.18\textwidth]{figures/Spectral_clustering/10cluster_SO3/Bispec_0_16.eps}}
     \end{tabular}
     \caption{Spectral clustering result with $K = 10$ clusters and SO(3) group transformation at different SNRs. The affinities are estimated by . We have $n = 250$ number of points and each cluster has 25 points.}
     \label{fig:10_cluster_plot_SO3}
\end{figure}


==> textfiles/report.tex <==
\section{Method on SO(2)}
In this section we discuss about the SO(2) case. Given $n$ points lie on 2-D sphere with transformations SO(2), the affinity matrix $W_k$ at frequency $k$ is built as:
\begin{equation}
    W_k(i, j) = 
    \begin{cases} 
    w_{ij}e^{\imath k\alpha_{ij}} &(i, j) \in E, \\ 
    0 &\text{otherwise},
    \end{cases}
\label{eq:Wk}
\end{equation}
where $w_{ij} = w_{ji}$ and $\alpha_{ij} = -\alpha_{ji}$ for all $ (i,j) \in E$. At frequency $k$, the weighted degree of node $i$ is:
\begin{equation}
    \mathrm{deg}(i) : = \sum_{j: (i,j) \in E}|W_k(i, j)| = \sum_{j: (i,j) \in E} w_{ij},
\end{equation}
and the degree is identical through all frequencies. We define a diagonal degree matrix $D$ of size $n\times n$, where the $i^{\text{th}}$ diagonal entry $D(i,i) = \mathrm{deg}(i)$. Then the operator $A_k = D^{-1}W_k$ is used to describe a Markov Chain, where $A_k(i,j)$ represents the transition probability from node $i$ to $j$ in a single step. Moreover, if we use $2t$ random walk steps, $A^{2t}_k(i,j)$ is the probability from $i$ to $j$ that includes all possible paths with length $2t$. Clearly, large $|A^{2t}_k(i,j)|$ indicates a close connection between $i$ and $j$.
\subsection{MFVDM affinity}
Intuitively, we could use $|A^{2t}_k(i,j)|$ to quantify the affinity between $(i,j)$. Moreover, we have the following observation:
\begin{equation}
    A_{k} = D^{-1}W_{k} = D^{-1/2} \underbrace{D^{-1/2}W_{k}D^{-1/2}}_{S_{k}} D^{1/2}.
    \label{eq:A_k}
\end{equation}
Since $S_k$ is Hermition, we compute $S_k^{2t}(i,j)$ instead of $A_k^{2t}(i,j)$. $S_k$ can be eigen-decompsed as:
\begin{align}
    S_{k}^{2t}(i, j) &= \sum_{l = 1}^{n}\left(\lambda_{l}^{(k)}\right)^{2t} u_{l}^{(k)}(i)\overline{u_{l}^{(k)}(j)},
    \label{eq:eigen_decom}
\end{align}
where $\lambda_{1}^{(k)} > \lambda_{2}^{(k)} > \ldots >\lambda_{n}^{(k)}$. Therefore the affinity between $i$ and $j$ at the $k^{\text{th}}$ frequency is given by
\begin{align}
|S_{k}^{2t}(i,j)|^2 & = \sum_{l,r = 1}^{n}\left(\lambda_{l}^{(k)}\lambda_{r}^{(k)}\right)^{2t}u_{l}^{(k)}(i) \overline{u_{r}^{(k)}(i)} \overline{u_{l}^{(k)}(j)} u_{r}^{(k)}(j) \nonumber \\
     &= \left\langle V_t^{(k)}(i), V_t^{(k)}(j)\right\rangle,
     \label{eq:affinity_k_untrun}
\end{align}
which is expressed by an inner product between two vectors $V^{(k)}_t(i), V^{(k)}_t(j) \in \mathbb{C}^{n^2}$ via the mapping $V_{t}^{(k)}$:
\begin{equation}
    V_{t}^{(k)}: i \mapsto \left(\left(\lambda_{l}^{(k)}\lambda_{r}^{(k)}\right)^t \langle u_{l}^{(k)}(i), u_{r}^{(k)}(i) \rangle \right)_{l,r = 1}^n. 
\end{equation}

\noindent\textbf{Truncated mapping}:
Notice the matrices $I + S_k$ and $I - S_k$ are both positive semi-definite (PSD) due to the following property: $\forall v \in \mathbb{C}^n$ we have 
\begin{align}
    &v^{*}(I \pm S_k)v = \\
    &\sum_{(i,j) \in E} w_{ij}\left | \frac{v(i)}{\sqrt{\deg{(i)}}} \pm \frac{ e^{\imath k\alpha_{ij}}v(j)}{\sqrt{\deg(j)}} \right |^2 \geq 0. \nonumber
\end{align}
Therefore all eigenvalues $\{\lambda^{(k)}_i\}_{i = 1}^{n}$ of $S_k$  lie within the interval $[-1,1]$.
Consequently, for large $t$, most  $(\lambda_{l}^{(k)}\lambda_{r}^{(k)})^{2t}$ terms in Eq.~\eqref{eq:affinity_k_untrun} are close to 0, and $|S_k^{2t}
(i, j) |^2$  can be well  approximated by using only a few of the 
largest eigenvalues and their corresponding eigenvectors. Hence, we truncate the frequency-$k$-VDM mapping $V_{t}^{(k)}$ using a cutoff $m_k$ for each frequency $k$: 
\begin{equation}
    \hat{V}_{t}^{(k)}: i \mapsto \left(\left(\lambda_{l}^{(k)}\lambda_{r}^{(k)}\right)^t \langle u_{l}^{(k)}(i), u_{r}^{(k)}(i) \rangle \right)_{l,r = 1}^{m_k}.
    \label{eq:trun_V}
\end{equation}
The affinity for each $k$ after truncation is given by
\begin{equation}
    |\hat{S}_{k}^{2t}(i, j)|^2 = \left\langle \hat{V}_{t}^{(k)}(i), \hat{V}_{t}^{(k)}(j) \right\rangle \approx |S_k^{2t}(i,j)|^2.
\end{equation}

\noindent
\textbf{Multi-frequency mapping}: 
Consider the affinity in Eq.~\eqref{eq:affinity_k_untrun} for $k = 1,\ldots, k_{\text{max}}$. If $i$ and $j$ are connected by paths with consistent transformation, the affinity $|\hat{S}_{k}^{2t}(i, j)|^2$ is large for all $k$. We can combine multiple representations on the same graph to evaluate the consistencies of group transformation along connected paths. Therefore, we define the extended mapping $\hat{V}_{t}$ as a concatenation of the truncated mappings $\hat{V}_{t}^{(k)}$ that $\forall k$:
\begin{equation}
    \hat{V}_{t}(i): i \mapsto \left(\hat{V}_{t}^{(1)}(i); \hat{V}_{t}^{(2)}(i); \ldots;\hat{V}_{t}^{(k_{\text{max}})}(i) \right).
    \label{eq:MFVDM_map}
\end{equation}
Then the total affinity of $i$ and $j$ is the inner product of $\hat{V}_{t}(i)$ and $\hat{V}_{t}(j)$:
\begin{align}
|\hat{S}^{2t}_{\text{MFVDM}}(i,j)|^2 :&= \sum_{k = 1}^{k_\text{max}}|\hat{S}_k^{2t}(i,j)|^2 = \sum_{k = 1}^{k_\text{max}}\left\langle \hat{V}_t^{(k)}(i), \hat{V}_t^{(k)}(j)\right\rangle \nonumber \\
      &  =  \left\langle \hat{V}_{t}(i), \hat{V}_{t}(j) \right\rangle.
      \label{eq:affinity_total}        
\end{align}
We call this \textbf{Multi-frequency VDM(MFVDM) affinity}, which is an extention of VDM.

\subsection{Optimal alignment affinity}
We notice that the eigenvectors of $S_k$ encode the alignment information between neighboring nodes, as illustrated in Fig.~\ref{fig:eVDM_align}. Assume that two nodes $i$ and $j$ are located at the same base manifold point, for example, the same point on $S^2$, but their tangent bundle frames are oriented differently, with an in-plane rotational angle $\alpha_{ij}$. Then the corresponding entries of eigenvalues are vectors in the complex plane and the following holds, 
\begin{equation}
u^{(k)}_{l}(i) = e^{\imath k \alpha_{ij}} u^{(k)}_l(j), \quad \forall\, l = 1,2,\ldots,n.
\label{eq:sameview}
\end{equation}
When $i$ and $j$ are close but not identical, Eq.~\eqref{eq:sameview} holds approximately for each frequency $k$. Therefore we propose another affinity by inspecting this consistency along frequency $k$ as:
\begin{align}
|\hat{S}^{2t}_{\text{OA}}(i,j)| :&= \min_\alpha \sum_{k = 1}^{ k_{\text{max}} } \sum_{l = 1}^{m_k} \left(\lambda_l^{(k)}\right)^{2t} \left| u^{(k)}_l(i) - e^{\imath k \alpha} u^{(k)}_l(j) \right|^2 \nonumber \\
& = \max_\alpha \sum_{k = 1}^{ k_{\text{max}} } \left( \sum_{l = 1}^{m_k} \left(\lambda_l^{(k)}\right)^{2t} u_l^{(k)}(i) \overline{u_l^{(k)}(j)}\right) e^{-\imath k \alpha} \nonumber\\
&= \max_\alpha \sum_{k = 1}^{ k_{\text{max}} }\hat{S}^{2t}_k(i.j)e^{-ik\alpha}.  
\label{eq:EVDMalign2}
\end{align}
Notice we apply the similar truncation idea on the eigenvectors as above and use $\hat{S}^{2t}_k$ to represent it. To solve Eq.~(\ref{eq:EVDMalign2}), we define a sequence $v$ and set $v(k)$ for $k = 1, 2, \dots, k_\text{max}$ to be
%Benefits from the irreducible representation $k$, we could use Fast Fourier Transform(FFT) to find a solution for Eq.(\ref{eq:EVDMalign2}) efficiently, as taking a length $N$ sequence $u$ that:
\begin{equation}
    v(k) =  \hat{S}^{2t}_k(i.j) = \sum_{l = 1}^{m_k} \left(\lambda_l^{(k)}\right)^{2t} u_l^{(k)}(i) \overline{u_l^{(k)}(j)}.
    \label{eq:u}
\end{equation}
When comparing Eq.~\eqref{eq:u} with Eq.~\eqref{eq:EVDMalign2}, it's obvious that the alignment angles $\hat{\alpha}_{ij}$ can be efficiently estimated by using an FFT on zero-padded $v$ and identifying its peak, we call this \textbf{optimal alignment(OA) affinity}. Comparing with the MFVDM affinity, the optimal alignment affinity include the consistency along different frequency $k$, which could furthermore enhance its robustness to noise.

\subsection{Bispectrum affinity}
The main drawback for the optimal alignment affinity is that, computing $|S^{2t}_k(i.j)|$ for each $(i,j)$ is computation consuming, also finding the peak of FFT could induce error when it is non-convex with $\alpha$. Therefore, another way to inspect the consistency between different frequency $k$ is  bispectrum, \yifeng{Not sure how to introduce the bispectrum here} where for the $l^{\text{th}}$ eigenvector on two frequencies $k_1, k_2$, the bispectrum term is built as:
\begin{equation}
    u_l^{(k_1)}(i)u_l^{(k_2)}(i)\overline{u_l^{(k_1 -k_2)}(i)}
\end{equation}

For frequency $k_1$ and $k_2$, the \textbf{bispectrum(Bisp) affinity} between $(i,j)$ is given as:
\begin{equation}
    \hat{S}_{k_1,k_2, k_3 = k_1 - k_2}^{2t}(i,j)_{\text{bisp}} = \sum_{l_1}^{m_{k_1}}\sum_{l_2}^{m_{k_2}}\sum_{l_3}^{m_{k_3}}(\lambda_{l_1}^{(k_1)}\lambda_{l_2}^{(k_2)}\lambda_{l_3}^{(k_3)})^{2t}
    u_{l_1}^{(k_1)}(i)u_{l_2}^{(k_2)}(i)u_{l_3}^{(k_3)}(i)\overline{u_{l_1}^{(k_1)}(j)u_{l_2}^{(k_2)}(j)u_{l_3}^{(k_3)}(j)},
\end{equation}
then the total affinity is given as:
\begin{equation}
    \hat{S}^{2t}_{\text{bisp}}(i,j) = \sum_{k_1}^{k_{\text{max}}}\sum_{k_2}^{k_{\text{max}}}\hat{S}^{2t}_{k_1,k_2, k_3 = k_2 - k_1}(i,j)_{\text{bisp}}.
\end{equation}
Similarly, the bispectrum mapping is given as:
\begin{equation}
    \hat{V}_{t, \text{Bisp}} : i \mapsto \left(\lambda_{l_1}^{(k_1)}\lambda_{l_2}^{(k_2)}\lambda_{l_3}^{(k_1 - k_2)}\right)^t u_{l_1}^{(k_1)}(i)u_{l_2}^{(k_2)}(i)u_{l_3}^{(k_1 - k_2)}(i).
\end{equation}
Similar to the MFVDM affinity, bispectrum affinity is also rotational invariant, and could be more robust to noise by including the consistency among different frequency $k$.

\subsection{Normalization on eigenvectors}
Empirically we find normalization on eigenvectors help to identify nearest neighbors. As shown in Eq.~\eqref{eq:eigen_decom}, for each node $i$ we concatenate the $i^{\text{th}}$ entry for the $l = 1, \ldots, m_k$ at frequency $k$, which is denoted as $\{u_l^{(k)}(i)\}_{l = 1}^{m_k}$, and the normalization is to replace $u_l^{(k)}(i)$ by $\frac{u_l^{(k)}(i)}{\|\{u_l^{(k)}(i)\}_{l = 1}^{m_k}\|}$ in Eq.~\eqref{eq:eigen_decom}.


\subsection{Algorithms and computational complexity}
The algorithms for the three affinity approaches are summarized in Alg.~\ref{alg:MFVDM_affinity},~\ref{alg:OA_affinity},~\ref{alg:Bisp_affinity}, respectively. For the computational complexity, firstly computing the top $m_k$ eigenvectors of the sparse Hermitian matrices $S_k$, for $k = 1, \dots, k_{\text{max}}$ requires $O(\sum_{k = 1}^{k_{\text{max}}} n (m_k^2 + m_k l))$, where $l$ is the average number of non-zero elements in each row of $S_k$ (e.g. number of NNs). Next for computing the affinity. MFVDM takes $O(n^2\sum_{k = 1}^{k_{\text{max}}}m_k^2)$. For optimal alignment affinity, suppose we use $N$-point FFT, then it costs $O(n^2(\sum_{k = 1}^{k_{\text{max}}}m_k + N\log N)$. We summarize the computational complexity in Tab.~\ref{tab:complexity_affinity}. Notice that usually $n \gg m_k$ for all $k$ and $n \gg l$, then the complexity is dominated by the second part.

\begin{table}[t!]
    \centering
    \scriptsize
    \caption{Computational complexity for three affinity approaches. (1): Eigen-decomposition on sparse Hermition matrix $S_k$ for $k = 1,\ldots,k_{\text{max}}$. (2): Computing the affinities for all $(i,j)$ pairs.}
    \vspace{0.1cm}
    \begin{tabular}{p{0.07\textwidth}<{\centering}|p{0.25\textwidth}<{\centering}|p{0.25\textwidth}<{\centering}|p{0.25\textwidth}<{\centering}} \toprule
     Steps &MFVDM &Optimal alignment &Bispectrum\\ \midrule
     (1) &\multicolumn{3}{c}{$O(n\sum_{k = 1}^{k_{\text{max}}} (m_k^2 + m_k l))$}\\ \midrule
     (2) &$O(n^2\sum_{k = 1}^{k_{\text{max}}}m_k^2)$ &$O(n^2(\sum_{k = 1}^{k_{\text{max}}}m_k + N\log N))$ & \\ \bottomrule
     
    \end{tabular}
    \label{tab:complexity_affinity}
\end{table}

\begin{algorithm}[t!]
\small
\SetAlgoLined
\SetAlTitleFnt{\footnotesize}
\SetAlCapNameFnt{\footnotesize}
\SetAlCapFnt{\footnotesize}
\KwIn{Initial noisy nearest neighbor graph $G = (V, E)$ and the corresponding edge weights $w^{(k)}_{ij}e^{\imath k\alpha_{ij}}$ defined on the edges, truncation cutoff $m_k$ for $k = 1, \dots, k_\text{max}$}
\KwOut{Affinity for all pair of nodes $(i,j)$}
\For{$k = 1, \dots, k_{\mathrm{max}} $}{
Construct the normalized affinity matrix $W_k$ and $S_k$ according to Eq.~\eqref{eq:Wk} and Eq.~\eqref{eq:A_k}\\
Compute the largest $m_k$ eigenvalues $\lambda^{(k)}_1 \geq \lambda^{(k)}_2, \geq, \dots, \geq \lambda^{(k)}_{m_k}$ of $S_k$ and the corresponding eigenvectors $\{ u^{(k)}_l \}_{l = 1}^{m_k}$ \\
(Optional): replace $u_l^{(k)}(i)$ by $\frac{u_l^{(k)}(i)}{\|\{u_l^{(k)}(i)\}_{l = 1}^{m_k}\|}$\\
Compute the truncated MFVDM embedding $\hat{V}^{(k)}_{t}$ according to Eq.~\eqref{eq:trun_V}
}
Concatenate the truncated embedding $\{\hat{V}^{(k)}_{t}\}_{k = 1}^{k_{\text{max}}}$ as Eq.~\ref{eq:MFVDM_map} and compute the affinity by Eq.~\eqref{eq:affinity_total}
\caption{MFVDM affinity}
\label{alg:MFVDM_affinity}
\end{algorithm}

\begin{algorithm}[t!]
\small
\SetAlgoLined
\SetAlTitleFnt{\footnotesize}
\SetAlCapNameFnt{\footnotesize}
\SetAlCapFnt{\footnotesize}
\KwIn{Initial noisy nearest neighbor graph $G = (V, E)$ and the corresponding edge weights $w^{(k)}_{ij}e^{\imath k\alpha_{ij}}$ defined on the edges, truncation cutoff $m_k$ for $k = 1, \dots, k_\text{max}$}
\KwOut{Affinity for all pair of nodes $(i,j)$}
\For{$k = 1, \dots, k_{\mathrm{max}} $}{
Construct the normalized affinity matrix $W_k$ and $S_k$ according to Eq.~\eqref{eq:Wk} and Eq.~\eqref{eq:A_k}\\
Compute the largest $m_k$ eigenvalues $\lambda^{(k)}_1 \geq \lambda^{(k)}_2, \geq, \dots, \geq \lambda^{(k)}_{m_k}$ of $S_k$ and the corresponding eigenvectors $\{ u^{(k)}_l \}_{l = 1}^{m_k}$ \\
(Optional): replace $u_l^{(k)}(i)$ by $\frac{u_l^{(k)}(i)}{\|\{u_l^{(k)}(i)\}_{l = 1}^{m_k}\|}$\\
}
\For{i = 1,\ldots, n}{\For{j = i+1,\ldots, n}{Compute the optimal alignment affinity for $(i,j)$ based on Eq.~\eqref{eq:EVDMalign2}}}
\caption{Optimal alignment affinity}
\label{alg:OA_affinity}
\end{algorithm}

\begin{algorithm}[t!]
\small
\SetAlgoLined
\SetAlTitleFnt{\footnotesize}
\SetAlCapNameFnt{\footnotesize}
\SetAlCapFnt{\footnotesize}
\KwIn{Initial noisy nearest neighbor graph $G = (V, E)$ and the corresponding edge weights $w^{(k)}_{ij}e^{\imath k\alpha_{ij}}$ defined on the edges, truncation cutoff $m_k$ for $k = 1, \dots, k_\text{max}$}
\KwOut{Affinity for all pair of nodes $(i,j)$}
\For{$k = 1, \dots, k_{\mathrm{max}} $}{
Construct the normalized affinity matrix $W_k$ and $S_k$ according to Eq.~\eqref{eq:Wk} and Eq.~\eqref{eq:A_k}\\
Compute the largest $m_k$ eigenvalues $\lambda^{(k)}_1 \geq \lambda^{(k)}_2, \geq, \dots, \geq \lambda^{(k)}_{m_k}$ of $S_k$ and the corresponding eigenvectors $\{ u^{(k)}_l \}_{l = 1}^{m_k}$ \\
(Optional): replace $u_l^{(k)}(i)$ by $\frac{u_l^{(k)}(i)}{\|\{u_l^{(k)}(i)\}_{l = 1}^{m_k}\|}$\\
}
Concatenate the truncated embedding $\{\hat{V}^{(k)}_{t}\}_{k = 1}^{k_{\text{max}}}$ and compute the affinity by Eq.~\eqref{eq:affinity_total}
\caption{Bispectrum affinity}
\label{alg:Bisp_affinity}
\end{algorithm}

\begin{algorithm}[t!]
\small
\SetAlgoLined
\SetAlTitleFnt{\footnotesize}
\SetAlCapNameFnt{\footnotesize}
\SetAlCapFnt{\footnotesize}
\KwIn{Initial noisy nearest neighbor graph $G = (V, E)$ and the corresponding edge weights $w^{(k)}_{ij}e^{\imath k\alpha_{ij}}$ defined on the edges, truncation cutoff $m_k$ for $k = 1, \dots, k_\text{max}$}
\KwOut{Affinity for all pair of nodes $(i,j)$}
\For{$k = 1, \dots, k_{\mathrm{max}} $}{
Construct the normalized affinity matrix $W_k$ and $S_k$ according to Eq.~\eqref{eq:Wk} and Eq.~\eqref{eq:A_k}\\
Compute the largest $m_k$ eigenvalues $\lambda^{(k)}_1 \geq \lambda^{(k)}_2, \geq, \dots, \geq \lambda^{(k)}_{m_k}$ of $S_k$ and the corresponding eigenvectors $\{ u^{(k)}_l \}_{l = 1}^{m_k}$ \\
(Optional): replace $u_l^{(k)}(i)$ by $\frac{u_l^{(k)}(i)}{\|\{u_l^{(k)}(i)\}_{l = 1}^{m_k}\|}$\\
Compute the truncated MFVDM embedding $\hat{V}^{(k)}_{t}$ according to Eq.~\eqref{eq:trun_V}
}
Concatenate the truncated embedding $\{\hat{V}^{(k)}_{t}\}_{k = 1}^{k_{\text{max}}}$ as Eq.~\ref{eq:MFVDM_map} and compute the affinity by Eq.~\eqref{eq:affinity_total}
\caption{MFVDM affinity}
\label{alg:MFVDM_affinity}
\end{algorithm}


\subsection{$\SO(2)$ rotational alignment}
\label{sec:SO2}
We assume the initial graph $G$ is given along with the optimal alignments on the connected edges. For simplicity and because of our interest in cryo-EM image classification, we focus on $\mathcal{G} = \SO(2)$ and we denote the optimal alignment angle by $\alpha_{ij}$. The corresponding frequency-$k$ unitary irreducible representations is $e^{\imath k \alpha_{ij}}$, where $\imath = \sqrt{-1}$. For points that are nearby on $\mathcal{M}$, the alignments should have cycle consistency under the clean case, for example, $k (\alpha_{ij} + \alpha_{jk} + \alpha_{ki}) \approx 0 \text{ mod } 2\pi $ for integers $k \in \mathbb{Z}$, if nodes $i$, $j$ and $k$ are true nearest neighbors. To systematically incorporate the alignment information and impose the consistency of alignments, for a given graph $G = (V, E)$, we construct a set of $n\times n$ affinity matrices $W_{k}$, 
\begin{equation}
    W_k(i, j) = 
    \begin{cases} 
    w_{ij}e^{\imath k\alpha_{ij}} &(i, j) \in E, \\ 
    0 &\text{otherwise},
    \end{cases}
\label{eq:Wk}
\end{equation}
where $w_{ij} = w_{ji}$ and $\alpha_{ij} = -\alpha_{ji}$ for all $ (i,j) \in E$. The degree of node $i$ is: $\mathrm{deg}(i) := \sum_{j: (i,j) \in E} w_{ij}$ and the degree matrix $D$ is a block diagonal matrix and the $(i, i)$ block of the matrix $D(i, i) = \mathrm{deg}(i) I_{d_k \times d_k}$. The degree is identical through all frequencies. We construct the normalized matrix $A_k = D^{-1}W_k$. The matrix $A_k$ is an averaging operator for vector fields, i.e.\ $(A_k z)(i) = \frac{1}{\mathrm{deg}(i)} \sum_{j: (i, j) \in E} w_{ij} \rho_k( z(j)$.

\paragraph{Optimal Alignment Affinity}
We notice that the eigenvectors of $S_k$ encode the alignment information between neighboring nodes, as illustrated in Fig.~\ref{fig:eVDM_align}. Assume that two nodes $i$ and $j$ are located at the same base manifold point, for example, the same point on $S^2$, but their tangent bundle frames are oriented differently, with an in-plane rotational angle $\alpha_{ij}$. Then the corresponding entries of eigenvalues are vectors in the complex plane and the following holds, 
\begin{equation}
u^{(k)}_{l}(i) = e^{\imath k \alpha_{ij}} u^{(k)}_l(j), \quad \forall\, l = 1,2,\ldots,n.
\label{eq:sameview}
\end{equation}
When $i$ and $j$ are close but not identical, Eq.~\eqref{eq:sameview} holds approximately for each frequency $k$. Therefore we propose another affinity by inspecting this consistency along frequency $k$ as:
\begin{align}
|\hat{S}^{2t}_{\text{OA}}(i,j)| :&= \min_\alpha \sum_{k = 1}^{ k_{\text{max}} } \sum_{l = 1}^{m_k} \left(\lambda_l^{(k)}\right)^{2t} \left| u^{(k)}_l(i) - e^{\imath k \alpha} u^{(k)}_l(j) \right|^2 \nonumber \\
& = \max_\alpha \sum_{k = 1}^{ k_{\text{max}} } \left( \sum_{l = 1}^{m_k} \left(\lambda_l^{(k)}\right)^{2t} u_l^{(k)}(i) \overline{u_l^{(k)}(j)}\right) e^{-\imath k \alpha} \nonumber\\
&= \max_\alpha \sum_{k = 1}^{ k_{\text{max}} }\hat{S}^{2t}_k(i.j)e^{-ik\alpha}.  
\label{eq:EVDMalign2}
\end{align}
Notice we apply the similar truncation idea on the eigenvectors as above and use $\hat{S}^{2t}_k$ to represent it. To solve Eq.~(\ref{eq:EVDMalign2}), we define a sequence $v$ and set $v(k)$ for $k = 1, 2, \dots, k_\text{max}$ to be
%Benefits from the irreducible representation $k$, we could use Fast Fourier Transform(FFT) to find a solution for Eq.(\ref{eq:EVDMalign2}) efficiently, as taking a length $N$ sequence $u$ that:
\begin{equation}
    v(k) =  \hat{S}^{2t}_k(i.j) = \sum_{l = 1}^{m_k} \left(\lambda_l^{(k)}\right)^{2t} u_l^{(k)}(i) \overline{u_l^{(k)}(j)}.
    \label{eq:u}
\end{equation}
When comparing Eq.~\eqref{eq:u} with Eq.~\eqref{eq:EVDMalign2}, it's obvious that the alignment angles $\hat{\alpha}_{ij}$ can be efficiently estimated by using an FFT on zero-padded $v$ and identifying its peak, we call this \textbf{optimal alignment(OA) affinity}. Comparing with the MFVDM affinity, the optimal alignment affinity include the consistency along different frequency $k$, which could furthermore enhance its robustness to noise.

Therefore, we can define the frequency-$k$ embedding for each node as
\begin{equation}
    \label{eq:node_embed_opt}
    V_k^{\text{opt}}(i) : i \mapsto \left [ \eta_t(\lambda_1) u_1^{(k)}, \eta_t(\lambda_2) u_2^{(k)}, \dots \eta_t(\lambda_n) u_n^{(k)}(i) \right]^\top, 
\end{equation}
Note that this embedding is not rotationally invariant, that is if we rotate the node by an angle $\alpha$, $V_k^{\text{opt}}(i) \mapsto V_k^{\text{opt}}(i) e^{\imath k \alpha}$. Combining multiple frequencies, the new similarity is defined as,
\begin{equation}
    \label{eq:sim_opt}
    S^{\text{opt}} (i, j) = \max_\alpha \mathrm{Re} \left [ \sum_{k = 1}^{k_\m } \left \langle  V_k^{\text{opt}}(i),  V_k^{\text{opt}}(i) \right \rangle  e^{\imath k \alpha} \right ],
\end{equation}
which can be approximated by zero-padded inverse fast Fourier transform.  

\paragraph{Invariant Feature Affinity and Embedding:}
The main drawback for the optimal alignment affinity is that, computing $|S^{2t}_k(i.j)|$ for each $(i,j)$ is computation consuming, also finding the peak of FFT could induce error when it is non-convex with $\alpha$. Therefore, another way to inspect the consistency between different frequency $k$ is  bispectrum, \yifeng{Not sure how to introduce the bispectrum here} where for the $l^{\text{th}}$ eigenvector on two frequencies $k_1, k_2$, the bispectrum term is built as:
\begin{equation}
    u_l^{(k_1)}(i)u_l^{(k_2)}(i)\overline{u_l^{(k_1 -k_2)}(i)}
\end{equation}

For frequency $k_1$ and $k_2$, the \textbf{bispectrum(Bisp) affinity} between $(i,j)$ is given as:
\begin{equation}
    \hat{S}_{k_1,k_2, k_3 = k_1 - k_2}^{2t}(i,j)_{\text{bisp}} = \sum_{l_1}^{m_{k_1}}\sum_{l_2}^{m_{k_2}}\sum_{l_3}^{m_{k_3}}(\lambda_{l_1}^{(k_1)}\lambda_{l_2}^{(k_2)}\lambda_{l_3}^{(k_3)})^{2t}
    u_{l_1}^{(k_1)}(i)u_{l_2}^{(k_2)}(i)u_{l_3}^{(k_3)}(i)\overline{u_{l_1}^{(k_1)}(j)u_{l_2}^{(k_2)}(j)u_{l_3}^{(k_3)}(j)},
\end{equation}
then the total affinity is given as:
\begin{equation}
    \hat{S}^{2t}_{\text{bisp}}(i,j) = \sum_{k_1}^{k_{\text{max}}}\sum_{k_2}^{k_{\text{max}}}\hat{S}^{2t}_{k_1,k_2, k_3 = k_2 - k_1}(i,j)_{\text{bisp}}.
\end{equation}
Similarly, the bispectrum mapping is given as:
\begin{equation}
    \hat{V}_{t, \text{Bisp}} : i \mapsto \left(\lambda_{l_1}^{(k_1)}\lambda_{l_2}^{(k_2)}\lambda_{l_3}^{(k_1 - k_2)}\right)^t u_{l_1}^{(k_1)}(i)u_{l_2}^{(k_2)}(i)u_{l_3}^{(k_1 - k_2)}(i).
\end{equation}
Similar to the MFVDM affinity, bispectrum affinity is also rotational invariant, and could be more robust to noise by including the consistency among different frequency $k$.

\subsection{Normalization on eigenvectors}
Empirically we find normalization on eigenvectors help to identify nearest neighbors. As shown in Eq.~\eqref{eq:eigen_decom}, for each node $i$ we concatenate the $i^{\text{th}}$ entry for the $l = 1, \ldots, m_k$ at frequency $k$, which is denoted as $\{u_l^{(k)}(i)\}_{l = 1}^{m_k}$, and the normalization is to replace $u_l^{(k)}(i)$ by $\frac{u_l^{(k)}(i)}{\|\{u_l^{(k)}(i)\}_{l = 1}^{m_k}\|}$ in Eq.~\eqref{eq:eigen_decom}.












